What Makes it Ok to Set a Fire? Iterative Self-distillation of Contexts and Rationales for Disambiguating Defeasible Social and Moral Situations

Moral or ethical judgments rely heavily on the specific contexts in which they occur. Understanding varying shades of defeasible contextualizations (i.e., additional information that strengthens or attenuates the moral acceptability of an action) is critical to accurately represent the subtlety and intricacy of grounded human moral judgment in real-life scenarios. We introduce defeasible moral reasoning: a task to provide grounded contexts that make an action more or less morally acceptable, along with commonsense rationales that justify the reasoning. To elicit high-quality task data, we take an iterative self-distillation approach that starts from a small amount of unstructured seed knowledge from GPT-3 and then alternates between (1) self-distillation from student models; (2) targeted filtering with a critic model trained by human judgment (to boost validity) and NLI (to boost diversity); (3) self-imitation learning (to amplify the desired data quality). This process yields a student model that produces defeasible contexts with improved validity, diversity, and defeasibility. From this model we distill a high-quality dataset, \delta-Rules-of-Thumb, of 1.2M entries of contextualizations and rationales for 115K defeasible moral actions rated highly by human annotators 85.9% to 99.8% of the time. Using \delta-RoT we obtain a final student model that wins over all intermediate student models by a notable margin.

==> tables/distill_algo.tex <==
% \begin{figure}[t]
% \begin{algorithm}[H]
% \footnotesize
% \caption{
%     Iterative Self-distillation of \datasetshort
% }


% \textbf{Input} initial policy model $\theta_0$, initial value model $\phi_0$, \delphi $\psi_{\text{Delphi}}$\\
%  \hspace*{2mm} $D_{\dataset} \gets$ Get dataset of clarification questions. \\
%   \hspace*{2mm} $\theta_{\text{Q}} \gets$ Fine-tune $\theta_0$ with Eqn~\ref{eqn:qgen_policy} from $D_{\text{\dataset}}$. \algorithmiccomment{Sec.~\ref{sec:policy}} \\
%    \hspace*{2mm} $D_{\dataset_{silver}} \gets$ Get silver dataset of defeasible answers to questions. \\
%      \hspace*{2mm} $\theta_{\text{A}} \gets$ Fine-tune lm with Eqn~\ref{eqn:agen_policy} from $D_{\text{\dataset}}$. \algorithmiccomment{Sec.~\ref{sec:answersim}} \\
%    \hspace*{2mm} $\theta_{\model{}} \gets$ \Call{ReinforcedLearning}{$S_{\text{SocialChem}}$, $\theta_{\text{Q}}$, $\theta_{\text{A}}$, $\phi_0$, $\psi_{\text{\delphi}}$} \\
% \hspace*{2mm} \phantom{...} \algorithmiccomment{Sec.~\ref{sec:rl}} 
% \begin{algorithmic}
% \Procedure{ReinforcedLearning}{$S_{\text{SocialChem}}$, $\theta_{\text{Q}}$, $\theta_{\text{A}}$, $\phi$, $\psi_{\text{\delphi}}$} 
%     \State $\theta_{Q_{\text{old}}} \gets \theta_Q$, $\phi_{\text{old}} \gets \phi$
%     \For{iterations = 1, 2, \ldots}
%         \State Sample a minibatch of situations $s$ from $S_{SocialChem}$.
%         \For{step = 1, 2, \ldots, $s$}
%             \State Calculate $r$ using $\theta_A$ and $\psi_{\text{Delphi}}$ with Eqn~\ref{eqn:reward}.
%             \State Compute $loss_{\text{PPO}}$ on the minibatch with Eqn~\ref{eqn:loss}.
%             \State Optimize $\theta$ and $\phi$ with $\mathcal{L}_{\text{PPO}}$ for one step.
%         \EndFor
%         \State $\theta_{Q_{\text{old}}} \gets \theta_Q$, $\phi_{\text{old}} \gets \phi$
%     \EndFor
%     \State \Return $\theta_Q$

    
% \EndProcedure
% \end{algorithmic}


% \textbf{Output} $\theta_{\model}$


% \label{alg:ppo}
% \end{algorithm}
% \end{figure}



% \begin{algorithm}[H]
%   \SetAlgoLined
%   \KwData{Input data}
%   \KwResult{Output result}

%   \BlankLine
%   \textbf{Initialization:} Initialize variables and data structures\;
  
%   \BlankLine
%   \textbf{Process data:} 
%   \For{each element in input data}{
%     Perform some operation\;
%     Update variables\;
%   }
  
%   \BlankLine
%   \textbf{Output result:} Output the final result\;

%   \caption{Example Algorithm}
% \end{algorithm}



\begin{algorithm}[H]
\footnotesize
\label{alg:iterative-self-distillation}
   \begin{algorithmic}[1]
   \Require teacher model $\tau$, critic model $\rho$, $A_{\text{SocialChem}}$
   \State $A_0 \gets$ sample $A_{\text{SocialChem}}$
   \State $A_{\text{SocialChem}} \gets A_{\text{SocialChem}} \setminus A_0$
   \State $D_0 \gets$ \Call{GenerateDiverse}{$\tau$, $A_0$}
   \State $D_0 \gets$ \Call{Filter}{$\rho$, $D_0$, $\text{Threshold}_{\text{distill}}$}
   \State $\textbf{Distill}_{base} \gets$ Fine-tune base model on $D_0$
   \For {$i = 1, 2$}
       \State $A_i \gets$ sample $A_{\text{SocialChem}}$
       \State $A_{\text{SocialChem}} \gets A_{\text{SocialChem}} \setminus A_i$
       \State $\textbf{SelfDistill}_i, D_i \gets$ \Call{SelfDistill}{$\sigma$, $A_i$, $\rho$} 
   \EndFor
   \State $D_{\text{rem}} \gets$ \Call{GenerateDiverse}{$\sigma$, $A_{\text{SocialChem}}$}
   \State return \Call{Filter}{$\rho$, $D_0 \cup D_1 \cup D_2 \cup D_{\text{rem}}$, $\text{Threshold}_{\text{dataset}}$}
   \Procedure{SelfDistill}{$\sigma_{\text{old}}$, $A$, $\rho$}
        \State $D \gets$ \Call{GenerateDiverse}{$\sigma$, $A$}
        \State $D_f \gets$ \Call{Filter}{$\rho$, $D$, $\text{Threshold}_{\text{distill}}$}
        \State $\sigma_{\text{new}} \gets$ Fine-tune $\sigma_{\text{old}}$ on $D_f$
        \State return $\sigma_{\text{new}}$, $D_f$
   \EndProcedure

   % \Procedure{GenerateDiverse}{$\mu$, $A$}
   %      \State $D \gets \emptyset$
   %      \For {$a$ in $A$}
   %          \For {$p = +, -$}
   %              \State $b \gets$ \{Top 10 beams from $\mu_{\text{old}}$ for $a, p$ \}
   %              \State $D_b \gets \emptyset$
   %              \For {$(a, p, c, r)$ in $b$}
   %                  \If {$\forall c' \in D_b: \lnot \Call{MutualNLI}{c, c'}$}
   %                      \State $D_b \gets D_b \cup \{ (a, p, c, r) \}$
   %                  \EndIf
   %              \EndFor
   %              \State $D \gets D \cup D_b$
   %          \EndFor
   %      \EndFor
   %      \State return $D$
   %  \EndProcedure
   
   % \Procedure{Filter}{$\rho$, $D$, $\kappa$}
   %      $D_f \gets \emptyset$
   %      \For {$(a, p, c, r)$ in $D$}
   %          \If {$\rho(a, p, c) > \kappa$}
   %              \State $D_f \gets D_f \cup \{ (a, p, c, r) \}$
   %          \EndIf
   %      \EndFor
   %      \State return $D_f$
   %  \EndProcedure

   % \Procedure{MutualNLI}{$c1$, $c2$}
   %      \State return $\text{Entail}(c1, c2) \land \text{Entail}(c2, c1)$
   % \EndProcedure

    \end{algorithmic}
\caption{Iterative Self-distillation of \datasetshort (full version in Appendix \ref{asec:full-algo})}
\end{algorithm}



==> tables/model_desc.tex <==
\begin{table}[b]
\small
\centering
    \begin{tabular}{ |c|c|c|c|c|c|c| }
        \hline
        Model & Base Model & Data Source & Decoding & Train Dataset Size & Critic Filter & NLI Filter \\
        \hline
        model-0.0.0 & flan-t5-xl & text-davinci-003 & n/a & 85K & yes & n/a \\
        \hline
        model-0.0.1 & flan-t5-xl & text-davinci-003 & n/a & 143K & no & n/a \\
        \hline
        model-0.0.2 & flan-t5-xl & text-davinci-003 & n/a & 67K & yes & n/a \\
        \hline
        model-1.0.0 & model-0.0.0 & model-0.0.0 & greedy & 53K & yes & n/a \\
        \hline
        model-1.1.0 & model-0.0.0 & model-0.0.0 & beam & 434K & yes & mutual \\
        \hline
        model-1.2.0 & model-0.0.0 & model-0.0.0 & beam & 326K & yes & one-way \\
        \hline
        model-1.1.1 & model-0.0.0 & model-0.0.0 & beam & 492K & yes & none \\
        \hline
        model-1.1.2 & model-0.0.0 & model-0.0.0 & beam & 869K & yes & mutual \\
        \hline
        model-2.1.0 & model-1.1.0 & model-1.1.0 & beam & 454K & yes & mutual \\
        \hline
    \end{tabular}
    \caption{Model experiment configurations.}
\label{tab:model-desc}
\end{table}

